Detection of Hidden Attacks on Cyber-Physical Systems from Serial Magnitude and Sign Randomness Inconsistencies

Stealthy false data injection attacks on cyber-physical systems (CPSs) introduce erroneous measurement information to on-board sensors with the purpose to degrade system performance. An intelligent attacker is able to leverage knowledge of the system model and noise characteristics to alter sensor measurements while remaining undetected. To achieve this objective, the stealthy attack sequence is designed such that the detector performs similarly in the attacked and attack-free cases. Consequently, an attacker that wants to remain hidden will leave behind traces of inconsistent behavior, contradicting the system model. To deal with this problem, we propose a runtime monitor to find these inconsistencies in sensor measurements by monitoring for serial inconsistencies of the detection test measure. Specifically, we employ the chi-square fault detection procedure to monitor the magnitude and signed sequence of its chi-square test measure. We validate our approach with simulations on an unmanned ground vehicle (UGV) under stealthy attacks and compare the detection performance with various state-of-the-art anomaly detectors.

==> HiddenAttacks.tex <==
\begin{section}{Hidden Attacks Background}
\label{sec:HiddenAttacks}


\textit{\;Zero-alarm attacks:} are attack sequences designed by an attacker that maintains the test measure from exceeding the defined threshold value ($z_k \leq \tau_z$). This class of attack does not trigger an alarm throughout the attack sequence, as the test measure never passes the threshold. In order to satisfy such requirements, an attacker must satisfy the attack vector by
\begin{equation} \label{eq:zero_alarm_attack}
    \bm{\xi}_k = -\bm{C}\bm{e}_k - \bm{\eta}_k + \bm{\Sigma}^{\frac{1}{2}} \bm{\delta}_k,
\end{equation}
where $\bm{\delta}_k \in \R^s$ is a vector that satisfies $\bm{\delta}_k^{\mathsf{T}}\bm{\delta}_k \leq \tau_z$. With this attack vector designed at a time $k$, the test measure $z_k$ results in
\begin{equation} \label{eq:zero_alarm_attack2}
\begin{split}
    z_k &= (\Tilde{\bm{y}}_k - \bm{C}\hat{\bm{x}}_k)^{\mathsf{T}} \bm{\Sigma}^{-1} (\Tilde{\bm{y}}_k - \bm{C}\hat{\bm{x}}_k) \\
    &= (\bm{C}\bm{e}_k + \bm{\eta}_k + \bm{\xi}_k)^{\mathsf{T}} \bm{\Sigma}^{-1} (\bm{C}\bm{e}_k + \bm{\eta}_k + \bm{\xi}_k) \leq \tau_z,
\end{split}
\end{equation}
that remains within the threshold value to not trigger an alarm. While generating an attack sequence that does not trigger alarms may seem like a favorable attack design to remain hidden from detection, it is necessary to recall that alarms are triggered in a system operating in normal conditions without attacks. If alarms are no longer being triggered as designed for in an attack-free case, then these conditions may raise suspicions of a possible attack. To avoid these alarm rate discrepancies, an attacker would want to design an attack sequence that is undetectable to emulate normal (attack-free) conditions. This class of attack brings us to develop a sequence that exploits the system uncertainties to execute such a malicious attack.

\textit{\;Hidden attacks:} can be defined as designed attack sequences such that alarms are triggered at the same rate as the desired false alarm rate during nominal, attack-free operation. As shown in Fig. \ref{fig:HiddenAttack}, during a hidden attack, a smart attacker can design sequence where the test measure $z_k$ exceeds the threshold $\tau_z$ at the same rate as the nominal case. Formally, the attack sequence with the vector $\bm{\delta}_k$ from \eqref{eq:zero_alarm_attack} is designed such that
\begin{equation} \label{eq:hidden_attack}
    \mathrm{Pr}(z_k > \tau_z) = \mathrm{Pr}(\bm{\delta}_k^{\mathsf{T}} \bm{\delta}_k > \tau_z) = \alpha,
\end{equation}
to remain hidden from detection.

\begin{figure}[th!b]
\centering
\includegraphics[width=0.45\textwidth]{Figures/HiddenAttack_PDF.png}
\caption{(top) The nominal chi-square distribution of $z_k$ with $s = 4$ degrees of freedom in the absence of sensor attacks. With a correctly chosen threshold value $\tau_z$, the random variable $z_k$ exceeds the threshold (i.e., $z_k > \tau_z$) at a desired alarm rate of $\alpha$ in the attack-free case. Similarly, during a hidden attack (bottom), an attacker can choose an attack vector $\bm{\xi}_k \ne 0$ sequence such that the alarm rate matches the desired alarm rate $\alpha$, all while altering the distribution of $z_k$ and remaining hidden from detection.}
\label{fig:HiddenAttack}
\end{figure}




\end{section}
